The eXtreme Mesh deformation approach (X-MESH) for the Stefan phase-change model

The eXtreme Mesh deformation approach (X-MESH) is a new paradigm to follow sharp interfaces without remeshing and without changing the mesh topology. Even though the mesh does not change its topology, it can follow interfaces that do change their topology (nucleation, coalescence, splitting). To make this possible, the key X-MESH idea is to allow elements to reach zero measure. This permits interface relaying between nodes as well as interface annihilation and seeding in a time continuous manner. The paper targets the Stefan phase change model in which the interface (front) is at a given temperature. Several examples demonstrate the capability of the approach.

==> conco.tex <==
% This file defines new characters to be used in Latex files 
% -------------------------------------------------------------------
%
% -------------------------------------------------------------------
% Bold letters in math style
% -------------------------------------------------------------------
\newcommand{\bfa}{\mbox{\boldmath $a$}}
\newcommand{\bfb}{\mbox{\boldmath $b$}}
\newcommand{\bfc}{\mbox{\boldmath $c$}}
\newcommand{\bfd}{\mbox{\boldmath $d$}}
\newcommand{\bfe}{\mbox{\boldmath $e$}}
\newcommand{\bff}{\mbox{\boldmath $f$}}
\newcommand{\bfg}{\mbox{\boldmath $g$}}
\newcommand{\bfh}{\mbox{\boldmath $h$}}
\newcommand{\bfi}{\mbox{\boldmath $i$}}
\newcommand{\bfj}{\mbox{\boldmath $j$}}
\newcommand{\bfk}{\mbox{\boldmath $k$}}
\newcommand{\bfl}{\mbox{\boldmath $l$}}
\newcommand{\bfm}{\mbox{\boldmath $m$}}
\newcommand{\bfn}{\mbox{\boldmath $n$}}
\newcommand{\bfo}{\mbox{\boldmath $o$}}
\newcommand{\bfp}{\mbox{\boldmath $p$}}
\newcommand{\bfq}{\mbox{\boldmath $q$}}
\newcommand{\bfr}{\mbox{\boldmath $r$}}
\newcommand{\bfs}{\mbox{\boldmath $s$}}
\newcommand{\bft}{\mbox{\boldmath $t$}}
\newcommand{\bfu}{\mbox{\boldmath $u$}}
\newcommand{\bfv}{\mbox{\boldmath $v$}}
\newcommand{\bfw}{\mbox{\boldmath $w$}}
\newcommand{\bfx}{\mbox{\boldmath $x$}}
\newcommand{\bfy}{\mbox{\boldmath $y$}}
\newcommand{\bfz}{\mbox{\boldmath $z$}}
%
\newcommand{\bfA}{\mbox{\boldmath $A$}}
\newcommand{\bfB}{\mbox{\boldmath $B$}}
\newcommand{\bfC}{\mbox{\boldmath $C$}}
\newcommand{\bfD}{\mbox{\boldmath $D$}}
\newcommand{\bfE}{\mbox{\boldmath $E$}}
\newcommand{\bfF}{\mbox{\boldmath $F$}}
\newcommand{\bfG}{\mbox{\boldmath $G$}}
\newcommand{\bfH}{\mbox{\boldmath $H$}}
\newcommand{\bfI}{\mbox{\boldmath $I$}}
\newcommand{\bfJ}{\mbox{\boldmath $J$}}
\newcommand{\bfK}{\mbox{\boldmath $K$}}
\newcommand{\bfL}{\mbox{\boldmath $L$}}
\newcommand{\bfM}{\mbox{\boldmath $M$}}
\newcommand{\bfN}{\mbox{\boldmath $N$}}
\newcommand{\bfO}{\mbox{\boldmath $O$}}
\newcommand{\bfP}{\mbox{\boldmath $P$}}
\newcommand{\bfQ}{\mbox{\boldmath $Q$}}
\newcommand{\bfR}{\mbox{\boldmath $R$}}
\newcommand{\bfS}{\mbox{\boldmath $S$}}
\newcommand{\bfT}{\mbox{\boldmath $T$}}
\newcommand{\bfU}{\mbox{\boldmath $U$}}
\newcommand{\bfV}{\mbox{\boldmath $V$}}
\newcommand{\bfW}{\mbox{\boldmath $W$}}
\newcommand{\bfX}{\mbox{\boldmath $X$}}
\newcommand{\bfY}{\mbox{\boldmath $Y$}}
\newcommand{\bfZ}{\mbox{\boldmath $Z$}}
%
% -------------------------------------------------------------------
% Greek letters
% -------------------------------------------------------------------
\newcommand{\alp}{{\alpha}}
\newcommand{\bet}{{\beta}}
\newcommand{\gam}{{\gamma}}
\newcommand{\del}{{\delta}}
\newcommand{\eps}{{\epsilon}}
\newcommand{\vareps}{{\varepsilon}}
\newcommand{\zet}{{\zeta}}
\newcommand{\thet}{{\theta}}
\newcommand{\iot}{{\iota}}
\newcommand{\kap}{{\kappa}}
\newcommand{\lam}{{\lambda}}
\newcommand{\sig}{{\sigma}}
\newcommand{\ups}{{\upsilon}}
\newcommand{\ome}{{\omega}}
%
\newcommand{\Gam}{{\Gamma}}
\newcommand{\Del}{{\Delta}}
\newcommand{\Thet}{{\Theta}}
\newcommand{\Lam}{{\Lambda}}
\newcommand{\Sig}{{\Sigma}}
\newcommand{\Ups}{{\Upsilon}}
\newcommand{\Ome}{{\Omega}}
%
% -------------------------------------------------------------------
% Bold greek letters
% -------------------------------------------------------------------
\newcommand{\bfalp}{\mbox{\boldmath $\alpha$}}
\newcommand{\bfbet}{\mbox{\boldmath $\beta$}}
\newcommand{\bfgam}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfdel}{\mbox{\boldmath $\delta$}}
\newcommand{\bfeps}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bfvareps}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\bfvarphi}{\mbox{\boldmath $\varphi$}}
\newcommand{\bfzet}{\mbox{\boldmath $\zeta$}} 
\newcommand{\bfeta}{\mbox{\boldmath $\eta$}} 
\newcommand{\bfthet}{\mbox{\boldmath $\theta$}}
\newcommand{\bfiot}{\mbox{\boldmath $\iota$}}
\newcommand{\bfkap}{\mbox{\boldmath $\kappa$}}
\newcommand{\bflam}{\mbox{\boldmath $\lambda$}}
\newcommand{\bfmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bfnu}{\mbox{\boldmath $\nu$}}
\newcommand{\bfxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bfpi}{\mbox{\boldmath $\pi$}}
\newcommand{\bfrho}{\mbox{\boldmath $\rho$}}
\newcommand{\bfsig}{\mbox{\boldmath $\sigma$}}
\newcommand{\bftau}{\mbox{\boldmath $\tau$}}
\newcommand{\bfups}{\mbox{\boldmath $\upsilon$}}
\newcommand{\bfphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bfchi}{\mbox{\boldmath $\chi$}}
\newcommand{\bfpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\bfome}{\mbox{\boldmath $\omega$}}
%
\newcommand{\bfGam}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bfDel}{\mbox{\boldmath $\Delta$}}
\newcommand{\bfThet}{\mbox{\boldmath $\Theta$}}
\newcommand{\bfLam}{\mbox{\boldmath $\Lambda$}}
\newcommand{\bfXi}{\mbox{\boldmath $\Xi$}}
\newcommand{\bfPi}{\mbox{\boldmath $\Pi$}}
\newcommand{\bfSig}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bfUps}{\mbox{\boldmath $\Upsilon$}}
\newcommand{\bfPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bfPsi}{\mbox{\boldmath $\Psi$}}
\newcommand{\bfOme}{\mbox{\boldmath $\Omega$}}
%
% -------------------------------------------------------------------
% Letters with the tilde accents
% -------------------------------------------------------------------
\newcommand{\tia}{\tilde{a}}
\newcommand{\tib}{\tilde{b}}
\newcommand{\tic}{\tilde{c}}
\newcommand{\tid}{\tilde{d}}
\newcommand{\tie}{\tilde{e}}
\newcommand{\tif}{\tilde{f}}
\newcommand{\tig}{\tilde{g}}
\newcommand{\tih}{\tilde{h}}
\newcommand{\tii}{\tilde{i}}
\newcommand{\tij}{\tilde{j}}
\newcommand{\tik}{\tilde{k}}
\newcommand{\til}{\tilde{l}}
\newcommand{\tim}{\tilde{m}}
\newcommand{\tin}{\tilde{n}}
\newcommand{\tio}{\tilde{o}}
\newcommand{\tip}{\tilde{p}}
\newcommand{\tiq}{\tilde{q}}
\newcommand{\tir}{\tilde{r}}
\newcommand{\tis}{\tilde{s}}
\newcommand{\tit}{\tilde{t}}
\newcommand{\tiu}{\tilde{u}}
\newcommand{\tiv}{\tilde{v}}
\newcommand{\tiw}{\tilde{w}}
\newcommand{\tix}{\tilde{x}}
\newcommand{\tiy}{\tilde{y}}
\newcommand{\tiz}{\tilde{z}}
%
\newcommand{\wtiA}{\widetilde{A}}
\newcommand{\wtiB}{\widetilde{B}}
\newcommand{\wtiC}{\widetilde{C}}
\newcommand{\wtiD}{\widetilde{D}}
\newcommand{\wtiE}{\widetilde{E}}
\newcommand{\wtiF}{\widetilde{F}}
\newcommand{\wtiG}{\widetilde{G}}
\newcommand{\wtiH}{\widetilde{H}}
\newcommand{\wtiI}{\widetilde{I}}
\newcommand{\wtiJ}{\widetilde{J}}
\newcommand{\wtiK}{\widetilde{K}}
\newcommand{\wtiL}{\widetilde{L}}
\newcommand{\wtiM}{\widetilde{M}}
\newcommand{\wtiN}{\widetilde{N}}
\newcommand{\wtiO}{\widetilde{O}}
\newcommand{\wtiP}{\widetilde{P}}
\newcommand{\wtiQ}{\widetilde{Q}}
\newcommand{\wtiR}{\widetilde{R}}
\newcommand{\wtiS}{\widetilde{S}}
\newcommand{\wtiT}{\widetilde{T}}
\newcommand{\wtiU}{\widetilde{U}}
\newcommand{\wtiV}{\widetilde{V}}
\newcommand{\wtiW}{\widetilde{W}}
\newcommand{\wtiX}{\widetilde{X}}
\newcommand{\wtiY}{\widetilde{Y}}
\newcommand{\wtiZ}{\widetilde{Z}}
%
\newcommand{\tibfa}{\tilde{\bfa}}
\newcommand{\tibfb}{\tilde{\bfb}}
\newcommand{\tibfc}{\tilde{\bfc}}
\newcommand{\tibfd}{\tilde{\bfd}}
\newcommand{\tibfe}{\tilde{\bfe}}
\newcommand{\tibff}{\tilde{\bff}}
\newcommand{\tibfg}{\tilde{\bfg}}
\newcommand{\tibfh}{\tilde{\bfh}}
\newcommand{\tibfi}{\tilde{\bfi}}
\newcommand{\tibfj}{\tilde{\bfj}}
\newcommand{\tibfk}{\tilde{\bfk}}
\newcommand{\tibfl}{\tilde{\bfl}}
\newcommand{\tibfm}{\tilde{\bfm}}
\newcommand{\tibfn}{\tilde{\bfn}}
\newcommand{\tibfo}{\tilde{\bfo}}
\newcommand{\tibfp}{\tilde{\bfp}}
\newcommand{\tibfq}{\tilde{\bfq}}
\newcommand{\tibfr}{\tilde{\bfr}}
\newcommand{\tibfs}{\tilde{\bfs}}
\newcommand{\tibft}{\tilde{\bft}}
\newcommand{\tibfu}{\tilde{\bfu}}
\newcommand{\tibfv}{\tilde{\bfv}}
\newcommand{\tibfw}{\tilde{\bfw}}
\newcommand{\tibfx}{\tilde{\bfx}}
\newcommand{\tibfy}{\tilde{\bfy}}
\newcommand{\tibfz}{\tilde{\bfz}}
%
% -------------------------------------------------------------------
% Letters with hat accent
% -------------------------------------------------------------------
\newcommand{\whA}{\widehat{A}}
\newcommand{\whB}{\widehat{B}}
\newcommand{\whC}{\widehat{C}}
\newcommand{\whD}{\widehat{D}}
\newcommand{\whE}{\widehat{E}}
\newcommand{\whF}{\widehat{F}}
\newcommand{\whG}{\widehat{G}}
\newcommand{\whH}{\widehat{H}}
\newcommand{\whI}{\widehat{I}}
\newcommand{\whJ}{\widehat{J}}
\newcommand{\whK}{\widehat{K}}
\newcommand{\whL}{\widehat{L}}
\newcommand{\whM}{\widehat{M}}
\newcommand{\whN}{\widehat{N}}
\newcommand{\whO}{\widehat{O}}
\newcommand{\whP}{\widehat{P}}
\newcommand{\whQ}{\widehat{Q}}
\newcommand{\whR}{\widehat{R}}
\newcommand{\whS}{\widehat{S}}
\newcommand{\whT}{\widehat{T}}
\newcommand{\whU}{\widehat{U}}
\newcommand{\whV}{\widehat{V}}
\newcommand{\whW}{\widehat{W}}
\newcommand{\whX}{\widehat{X}}
\newcommand{\whY}{\widehat{Y}}
\newcommand{\whZ}{\widehat{Z}}
%
\newcommand{\ha}{\hat{a}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hc}{\hat{c}}
\newcommand{\hd}{\hat{d}}
\newcommand{\he}{\hat{e}}
\newcommand{\hf}{\hat{f}}
\newcommand{\hg}{\hat{g}}
\newcommand{\hh}{\hat{h}}
\newcommand{\hi}{\hat{i}}
\newcommand{\hj}{\hat{j}}
\newcommand{\hk}{\hat{k}}
\newcommand{\hl}{\hat{l}}
%\newcommand{\hm}{\hat{m}}
\newcommand{\hn}{\hat{n}}
\newcommand{\ho}{\hat{o}}
\newcommand{\hap}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hr}{\hat{r}}
\newcommand{\hs}{\hat{s}}
\newcommand{\htt}{\hat{t}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}
%
% -------------------------------------------------------------------
% Calligraphic letters
% -------------------------------------------------------------------
\newcommand{\ca}{{\cal A}}
\newcommand{\cb}{{\cal B}}
\newcommand{\cc}{{\cal C}}
\newcommand{\cd}{{\cal D}}
\newcommand{\ce}{{\cal E}}
\newcommand{\cf}{{\cal F}}
\newcommand{\cg}{{\cal G}}
\newcommand{\ch}{{\cal H}}
\newcommand{\ci}{{\cal I}}
\newcommand{\cj}{{\cal J}}
\newcommand{\ck}{{\cal K}}
\newcommand{\cl}{{\cal L}}
\newcommand{\cm}{{\cal M}}
\newcommand{\cn}{{\cal N}}
\newcommand{\co}{{\cal O}}
\newcommand{\cp}{{\cal P}}
\newcommand{\cq}{{\cal Q}}
\newcommand{\car}{{\cal R}}
\newcommand{\cs}{{\cal S}}
\newcommand{\ct}{{\cal T}}
\newcommand{\cu}{{\cal U}}
\newcommand{\cv}{{\cal V}}
\newcommand{\cw}{{\cal W}}
\newcommand{\cx}{{\cal X}}
\newcommand{\cy}{{\cal Y}}
\newcommand{\cz}{{\cal Z}}
%







==> macro.tex <==
% general
\newcommand{\erf}{\text{erf}}
\newcommand{\x}{\bm{x}}
\newcommand{\normalVect}{\bm{n}}

%pour le 2D
\newcommand{\xa}{\ensuremath{x_\mathrm{a}}}
\newcommand{\xb}{\ensuremath{x_\mathrm{b}}}
\newcommand{\xbb}{\ensuremath{\overline{x}_\mathrm{b}}}
\newcommand{\Kaa}{\ensuremath{K_\mathrm{aa}}}
\newcommand{\Kab}{\ensuremath{K_\mathrm{ab}}}
\newcommand{\Kba}{\ensuremath{K_\mathrm{ba}}}
\newcommand{\Kbb}{\ensuremath{K_\mathrm{bb}}}
\newcommand{\Kbbm}{\ensuremath{K_\mathrm{bb}^{-1}}}
\newcommand{\lb}{\ensuremath{\lambda_\mathrm{b}}}
\newcommand{\demi}{\ensuremath{\frac{1}{2}}}
\newcommand{\texton}{\text{\ on \ }}

\newcommand{\dertott}{\mathop{\frac{\mathrm{d}}{\mathrm{d}t}}}
\newcommand{\dint}{\mbox{\,  \ensuremath{\text{d}}}}
\newcommand{\jump}[1]{\mbox{$[\![ #1 ]\!]$}}
\newcommand{\tiT}{\tilde{T}}
\newcommand{\tilam}{\tilde{\lam}}
\newcommand{\Kred}{K_\mathrm{red}}
\newcommand{\Bleft}{B_\mathrm{left}}
\newcommand{\Gc}{G_\mathrm{c}}


% 1D stephan problem
\newcommand{\barLength}{L}
\newcommand{\Tmax}{T_{\text{max}}}
% \newcommand{\temp}{u}
% \newcommand{\test}{v}
\newcommand{\energy}{e}
\newcommand{\heatSource}{S}
\newcommand{\temp}{T}
\newcommand{\test}{\temp^*}
\newcommand{\tempDisc}{\temp_h}
\newcommand{\testDisc}{\test_h}
% \newcommand{\tempVect}{\bm{U}}
% \newcommand{\testVect}{\bm{V}}
\newcommand{\tempVect}{\bm{\temp}}
\newcommand{\testVect}{\bm{\test}}
\newcommand{\speed}{\bm{w}}
\newcommand{\speedVect}{\bm{\speed}}
\newcommand{\interfaceSpeed}{\speed_i}
\newcommand{\xnodes}{\bm{X}}
\newcommand{\fefunction}{\phi}
\newcommand{\OmegaS}{\Omega_s}
\newcommand{\OmegaL}{\Omega_\ell}
\newcommand{\front}{\Gamma}
\newcommand{\frontSpeed}{\bm{w}}
\newcommand{\volumicMass}{\rho}
\newcommand{\volumicMassSolid}{\volumicMass_s}
\newcommand{\volumicMassLiquid}{\volumicMass_\ell}
\newcommand{\specificHeat}{c}
\newcommand{\specificHeatSolid}{\specificHeat_s}
\newcommand{\specificHeatLiquid}{\specificHeat_\ell}
\newcommand{\conductivity}{k}
\newcommand{\conductivitySolid}{\conductivity_s}
\newcommand{\conductivityLiquid}{\conductivity_\ell}
\newcommand{\diffusivity}{\beta}
\newcommand{\diffusivitySolid}{\diffusivity_s}
\newcommand{\diffusivityLiquid}{\diffusivity_\ell}
\newcommand{\energyJump}{\bar{\ell}}
\newcommand{\latentHeat}{\ell}
\newcommand{\latentHeatVect}{\bm{\latentHeat}}
\newcommand{\specificHeatVect}{\bm{\specificHeat}}
\newcommand{\conductivityVect}{\bm{\conductivity}}
\newcommand{\energyJumpVect}{\bm{\energyJump}}
\newcommand{\phase}{\phi}
\newcommand{\phaseVect}{\bm{\phase}}
\newcommand{\updateMaterialProperties}{\text{UPDATE}}

% \newcommand{\dirichletBoundarySolid}{\partial_d \OmegaS}
% \newcommand{\dirichletBoundaryLiquid}{\partial_d \OmegaL}
\newcommand{\dirichletBoundary}{\Gamma^d}
\newcommand{\dirichletBoundarySolid}{\dirichletBoundary_s}
\newcommand{\dirichletBoundaryLiquid}{\dirichletBoundary_\ell}
\newcommand{\dirichletTemp}{\temp_d}
\newcommand{\boundaryTempSolid}{\temp_s}
\newcommand{\boundaryTempLiquid}{\temp_{\ell}}
\newcommand{\boundaryTempInterface}{\temp_{0}}
\newcommand{\initialTemp}{\temp_{i}}

\newcommand{\tempSpace}{\mathcal{U}}
\newcommand{\tempSpaceZero}{\tempSpace_0}

\newcommand{\frontPositionEx}{x_f}
\newcommand{\frontPositionExAxisym}{r_f}
\newcommand{\solexParam}{\phi}
\newcommand{\heatSink}{Q}

\newcommand{\meshSet}{\mathcal{M}}
\newcommand{\nodesSet}{\mathcal{N}}
\newcommand{\fe}{e}
\newcommand{\Nnodes}{N}
\newcommand{\elemSize}{h_e}
\newcommand{\timeStep}{\Delta t}
\newcommand{\mapping}{\mathcal{M}}
% \newcommand{\thalf}{\tfrac{1}{2}}
\newcommand{\thalf}{1/2}
\newcommand{\massMatrix}{\bm{M}}
\newcommand{\stiffnessMatrix}{\bm{K}}
\newcommand{\ALEMatrix}{\bm{L}}
\newcommand{\energyJumpMassRHS}{\bm{P}}
\newcommand{\energyJumpALERHS}{\bm{Q}}
\newcommand{\heatSourceRHS}{\bm{S}}
\newcommand{\interfaceID}{I}

\newcommand{\nstep}{n}
\newcommand{\nstepmax}{\nstep_{\text{max}}}
\newcommand{\niter}{k}
\newcommand{\nitermax}{\niter_{\text{max}}}
\newcommand{\err}{\text{err}}
\newcommand{\tol}{\text{tol}}
\newcommand{\tolT}{\tol_{\temp}}
\newcommand{\tolX}{\tol_{\xnodes}}
%% equations
\newcommand{\myeq}[2]{
\begin{equation}
\label{#2}
 #1
\end{equation}
}

\newcommand{\myeqalign}[1]{
\begin{align}
 #1
\end{align}
}

\newcommand{\eqspace}[0]{
 \; \;
}

\newcommand{\timeDeriv}[1]{
\ensuremath{ 
#1_{,t}
}
}

\newcommand{\myVectorGrad}[1]{
%  \overline{\overline{grad}} #1
   \ensuremath{ 
  \bm{\nabla} #1
  }
}

\newcommand{\myTranspose}[1]{
   \ensuremath{ 
 #1^{\top}
 }
}

\newcommand{\comment}[1]{
\textbf{(#1)}
}

